Learning Sample Reweighting for Accuracy and Adversarial Robustness

There has been great interest in enhancing the robustness of neural network classifiers to defend against adversarial perturbations through adversarial training, while balancing the trade-off between robust accuracy and standard accuracy. We propose a novel adversarial training framework that learns to reweight the loss associated with individual training samples based on a notion of class-conditioned margin, with the goal of improving robust generalization. We formulate weighted adversarial training as a bilevel optimization problem with the upper-level problem corresponding to learning a robust classifier, and the lower-level problem corresponding to learning a parametric function that maps from a sample's \textit{multi-class margin} to an importance weight. Extensive experiments demonstrate that our approach consistently improves both clean and robust accuracy compared to related methods and state-of-the-art baselines.

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section.~\ref{sec:limitations} in the Appendix.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Section.~\ref{sec:limitations} in the Appendix.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Code will be included as a link in the supplementary material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section.~\ref{sec:experiments}.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Section.~\ref{sec:experiments}}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See Section.~\ref{sec:experiments}.}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> figures/algorithms/reweighting_proc.tex <==
\begin{algorithm}[ht]
\caption{Sample reweighting}
\begin{flushleft}
\textbf{Input:} Training sample pairs $(X,y)$, validation sample pairs $(\hat{X}, \hat{y})$, classifier parameters $\theta_t$, sample weights $w_t$ \\
\textbf{Output:} $\nabla_\mu\hat{\mathcal{L}}_{\textrm{val}, w_t}|_{\theta_t}$ - gradient of the unweighted robust validation loss with respect to training sample weights $w$ evaluated at $\theta_t$ and $w_t$ 
\end{flushleft}
\begin{algorithmic}[1]
%\State Evaluate $\hat{\mathcal{L}}_{\textrm{tr}}|_{\theta_t,w_t}$ on $(X, y)$
\State $\tilde{\theta}_t \gets \theta_t - \beta\cdot\nabla_\theta\hat{\mathcal{L}}_\textrm{tr}|_{\theta_t, w_t}$
%\State Evaluate $\hat{\mathcal{L}}_{\textrm{val}}|_{\tilde{\theta}_t}$ on $(\hat{X}, \hat{y})$
\State Compute $\nabla_\mu\hat{\mathcal{L}}_{\textrm{val}}|_{\tilde{\theta},w_t}$ via backpropagation according to Eq. \ref{eq:wupdate}

\State \Return $\nabla_\mu\hat{\mathcal{L}}_{\textrm{val}}|_{\tilde{\theta}_t,w_t}$
\end{algorithmic}
\label{alg:reweighting_proc}
\end{algorithm} 

==> figures/pair-plot.tex <==
\begin{figure}
\includegraphics[trim={0 0.25cm 0 0},clip,width=0.24\textwidth]{figures/pair-plots/scale.png}
\includegraphics[width=0.24\textwidth]{figures/pair-plots-w/scale.png}
\includegraphics[trim={0 0.25cm 0 0},clip,width=0.24\textwidth]{figures/pair-plots/scale.png}
\includegraphics[width=0.24\textwidth]{figures/pair-plots-w/scale.png}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/airplane-automobile.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/airplane-automobile.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/airplane-bird.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/airplane-bird.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/airplane-cat.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/airplane-cat.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/airplane-deer.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/airplane-deer.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/airplane-dog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/airplane-dog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/airplane-frog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/airplane-frog.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/airplane-horse.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/airplane-horse.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/airplane-ship.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/airplane-ship.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/airplane-truck.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/airplane-truck.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/automobile-bird.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/automobile-bird.png}
%%%%%
\caption{\textbf{Part A} 2-d visualizations of the model’s output distribution of natural training data from two separated classes from CIFAR-10 dataset. The weight of a datum corresponds to the intesnity. of the color. The dark blue and dark red points represent samples with higher weight which are close to the class boundary; the light blue and light red points represent the samples with smaller weight. (Top colorbars corresponds to the $0-1$ normalized weights)}
\label{fig:weight_distribution}
\end{figure}

%%%%%%%%

\begin{figure}
\includegraphics[trim={0 0.25cm 0 0},clip,width=0.24\textwidth]{figures/pair-plots/scale.png}
\includegraphics[width=0.24\textwidth]{figures/pair-plots-w/scale.png}
\includegraphics[trim={0 0.25cm 0 0},clip,width=0.24\textwidth]{figures/pair-plots/scale.png}
\includegraphics[width=0.24\textwidth]{figures/pair-plots-w/scale.png}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/automobile-cat.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/automobile-cat.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/automobile-deer.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/automobile-deer.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/automobile-dog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/automobile-dog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/automobile-frog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/automobile-frog.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/automobile-horse.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/automobile-horse.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/automobile-ship.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/automobile-ship.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/automobile-truck.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/automobile-truck.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/bird-cat.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/bird-cat.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/bird-deer.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/bird-deer.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/bird-dog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/bird-dog.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/bird-frog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/bird-frog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/bird-horse.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/bird-horse.png}
\caption{\textbf{Part B} 2-d visualizations of the model’s output distribution on CIFAR-10 dataset.}
\end{figure}


%%%%%%%%

\begin{figure}
\includegraphics[trim={0 0.25cm 0 0},clip,width=0.24\textwidth]{figures/pair-plots/scale.png}
\includegraphics[width=0.24\textwidth]{figures/pair-plots-w/scale.png}
\includegraphics[trim={0 0.25cm 0 0},clip,width=0.24\textwidth]{figures/pair-plots/scale.png}
\includegraphics[width=0.24\textwidth]{figures/pair-plots-w/scale.png}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/bird-ship.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/bird-ship.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/bird-truck.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/bird-truck.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/cat-deer.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/cat-deer.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/cat-dog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/cat-dog.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/cat-frog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/cat-frog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/cat-horse.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/cat-horse.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/cat-ship.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/cat-ship.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/cat-truck.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/cat-truck.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/deer-dog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/deer-dog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/deer-frog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/deer-frog.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/deer-horse.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/deer-horse.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/deer-ship.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/deer-ship.png}
\caption{\textbf{Part C} 2-d visualizations of the model’s output distribution on CIFAR-10 dataset.}
\end{figure}


%%%%%

\begin{figure}
\includegraphics[trim={0 0.25cm 0 0},clip,width=0.24\textwidth]{figures/pair-plots/scale.png}
\includegraphics[width=0.24\textwidth]{figures/pair-plots-w/scale.png}
\includegraphics[trim={0 0.25cm 0 0},clip,width=0.24\textwidth]{figures/pair-plots/scale.png}
\includegraphics[width=0.24\textwidth]{figures/pair-plots-w/scale.png}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/deer-truck.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/deer-truck.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/dog-frog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/dog-frog.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/dog-horse.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/dog-horse.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/dog-ship.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/dog-ship.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/dog-truck.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/dog-truck.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/frog-horse.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/frog-horse.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/frog-ship.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/frog-ship.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/frog-truck.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/frog-truck.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/horse-ship.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/horse-ship.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/horse-truck.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/horse-truck.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/ship-truck.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/ship-truck.png}
\caption{\textbf{Part D} 2-d visualizations of the model’s output distribution on CIFAR-10 dataset.}
\end{figure}

==> figures/pair-plots-w/pair-plot.tex <==
\begin{figure}
\hspace*{0.4cm}\includegraphics[width=0.25\textwidth]{figures/pair-plots-w/scale.png}

\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/airplane-automobile.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/airplane-bird.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/airplane-cat.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/airplane-deer.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/airplane-dog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/airplane-frog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/airplane-horse.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/airplane-ship.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/airplane-truck.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/automobile-bird.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/automobile-cat.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/automobile-deer.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/automobile-dog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/automobile-frog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/automobile-horse.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/automobile-ship.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/automobile-truck.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/bird-cat.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/bird-deer.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/bird-dog.png}
%%%%%
\caption{\textbf{Part A} 2-d visualizations of the model’s output distribution of natural training data from two separated classes from CIFAR-10 dataset. The weight of a datum corresponds to the intesnity. of the color. The dark blue and dark red points represent samples with higher weight which are close to the class boundary; the light blue and light red points represent the samples with smaller weight. (Top colorbars corresponds to the $0-1$ normalized weights)}
\label{fig:weight_distribution}
\end{figure}

\begin{figure}
\hspace*{0.4cm}\includegraphics[width=0.25\textwidth]{figures/pair-plots-w/scale.png}

\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/bird-frog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/bird-horse.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/bird-ship.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/bird-truck.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/cat-deer.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/cat-dog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/cat-frog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/cat-horse.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/cat-ship.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/cat-truck.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/deer-dog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/deer-frog.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/deer-horse.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/deer-ship.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/deer-truck.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/dog-frog.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/dog-horse.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/dog-ship.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/dog-truck.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/frog-horse.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/frog-ship.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/frog-truck.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/horse-ship.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots-w/horse-truck.png}
\caption{\textbf{Part B} 2-d visualizations of the model’s output distribution on CIFAR-10 dataset. Samples colored by their assigned weight.}
\end{figure}


==> figures/pair-plots/pair-plot.tex <==
\begin{figure}

\hspace*{0.4cm}\includegraphics[width=0.25\textwidth]{figures/pair-plots/scale.png}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/airplane-automobile.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/airplane-bird.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/airplane-cat.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/airplane-deer.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/airplane-dog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/airplane-frog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/airplane-horse.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/airplane-ship.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/airplane-truck.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/automobile-bird.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/automobile-cat.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/automobile-deer.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/automobile-dog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/automobile-frog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/automobile-horse.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/automobile-ship.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/automobile-truck.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/bird-cat.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/bird-deer.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/bird-dog.png}
%%%%%
\caption{PCA applied to the model’s likelihood predictions on training samples of two classes from the CIFAR-10 dataset (horse \& deer). (\textbf{\subref{fig:plotbyk}}) The degree of robustness (denoted by the color gradient) of a data point is calculated based on the least number of iterations $\kappa$ that PGD needs to find its misclassified adversarial variant. (\textbf{\subref{fig:plotbyweight}}) The weight associated with the sample. (\textbf{\subref{fig:weight_distsf}}) Distribution of training sample weights learned by our method.}
\label{fig:robustness_distribution}
\end{figure}

\begin{figure}

\hspace*{0.4cm}\includegraphics[width=0.25\textwidth]{figures/pair-plots/scale.png}


\includegraphics[width=0.24\linewidth]{figures/pair-plots/bird-frog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/bird-horse.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/bird-ship.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/bird-truck.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/cat-deer.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/cat-dog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/cat-frog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/cat-horse.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/cat-ship.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/cat-truck.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/deer-dog.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/deer-frog.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/deer-horse.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/deer-ship.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/deer-truck.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/dog-frog.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/dog-horse.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/dog-ship.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/dog-truck.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/frog-horse.png}

\vspace{-0.5cm}

\includegraphics[width=0.24\linewidth]{figures/pair-plots/frog-ship.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/frog-truck.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/horse-ship.png}
\includegraphics[width=0.24\linewidth]{figures/pair-plots/horse-truck.png}
\caption{\textbf{Part B} 2-d visualizations of the model’s output distribution on CIFAR-10 dataset. Samples colored by $\kappa$, the number of PGD steps required to adversarially switch the example's label.}
\end{figure}

==> figures/tikz/meta_update.tex <==
\begin{figure}
\centering
\scalebox{0.8}{
      \begin{tikzpicture}[node distance=2.3cm]
        %\node[block, minimum height=2cm, text width=0.85cm,label={[align=left]above left:sample\\ weights}]                  (wt1){$w_{0,t-1}$ \\ $w_{1,t-1}$ \\ $w_{2,t-1}$ \\ \:\:\vdots \\ $w_{n,t-1}$};
        
        \node[block](wt_1){$w_{0,t-1}$};
        \node[block, below=0.55cm of wt_1](wt_2){$w_{1,t-1}$};
        \node[block, below=0.55cm of wt_2](wt_3){$w_{2,t-1}$};
        \node[block, below=0.55cm of wt_3](wt_4){$w_{3,t-1}$};
        
        \begin{scope}[on background layer]
        \node[fit={(wt_1) (wt_2)  (wt_3) (wt_4)}, draw,fill={blue!20},rounded corners] (wt1) {};
        \end{scope}
        
        \node[above of=wt1,scale=0.05](phant1){}; 
        
        
        \node[above =0.2cm of phant1,scale=0.05,label={above:{$\textcolor{blue}{w_t = \textrm{maml}(w_{t-1},\tilde{\theta})}$}}](phant12){};
        
        \node[above of=phant12,transform canvas={xshift=-1.2cm, yshift=-1.5cm}](phant12text){\textcolor{blue}{step 2:}};

        
        \node[left=1em of phant12,scale=0.05](phant13){};
        
        %\node[block, right of=wt1, minimum height=2cm, text width=0.85cm]                  (btr){$x_0$ \\ $x_1$ \\ $x_2$ \\ \:\:\vdots \\ $x_{b}$};
        \node[block, right of=wt1, minimum height=2cm, text width=0.85cm,label={[align=left]above right:training\\ samples}]                  (btr){\includegraphics[angle=0,origin=c,width=.85\textwidth]{figures/tikz/tr_set.png}};
        

        \node[block, right of=btr]   (tht){network \\ $\theta_{t-1}$};
        
        \node[right of=tht,scale=0.05,label={[yshift=0.1cm]above left:step 1}](phant2){};
        \node[above=0.5em of phant2,scale=0.05](phant22){};
        \node[below=0.5em of phant2,scale=0.05](phant23){};
        
        \node[block, right=1cm of phant2]   (gtr1){[weighted] loss \\ $\mathcal{L}_{\textrm{tr}}$};
        
        \node[below right =0.2cm of gtr1,transform canvas={xshift=0.5em}]   (tht1){$\textcolor{red}{\theta_t=GD(\theta_{t-1},\textcolor{blue}{w_t})}$};
        
        \node[above left = 0.05cm of tht1,transform canvas={xshift=1.2cm,yshift=-0.1cm}]   (tht12){\textcolor{red}{step 3:}};
        
        %\node[block, below =1cm of btr, minimum height=2cm, text width=0.85cm]                  (bval){$x_0$ \\ $x_1$ \\ $x_2$ \\ \:\:\vdots \\ $x_{b}$};
        %\node[block, below=1cm of btr, minimum height=2cm, text width=0.85cm,label={[align=left]above right:validation\\ samples}]                  (bval){\includegraphics[angle=0,origin=c,width=.85\textwidth]{figures/tikz/val_set.png}};
        
        \node[block, above right=1cm of gtr1, minimum height=2cm, text width=0.85cm,label={[align=left]above right:validation\\ samples}]                  (bval){\includegraphics[angle=0,origin=c,width=.85\textwidth]{figures/tikz/val_set.png}};
        
        \node[block, right of=bval]   (thtt){network \\ $\tilde{\theta}_t$};
        
        \node[below=2cm of thtt, scale=0.05, label={below right:$\tilde{\theta}=GD(\theta_{t-1},w_{t-1})$}]   (phant32){};
        \node[above=0.2cm of phant32, scale=0.05]   (phant33){};
        \node[left=0.2cm of phant33, scale=0.05]   (phant34){};
        \node[below=0.5cm of btr, scale=0.05]   (phant31){};

        \node[block, right=1cm of thtt]   (gtr2){unweighted loss \\ $\mathcal{L}_{\textrm{val}}$};
        
        
        
        %%%% boundaries
        \begin{scope}[on background layer]
            \node[draw,fit=(bval) (thtt) (gtr2),fill={gray},rounded corners, minimum height=4cm,text depth=0cm] (boundary1) {meta-update};
        \end{scope}
        %\path[line] (wt1) --          (gtr1);
        \path[-,draw]{} (wt1.north) --          (phant1);
        \path[line,rounded corners]{} (phant1) -|        (phant22);
        
        \path[line,transform canvas={xshift=-0.5em}, draw = blue]{} (phant12) --          (wt1.north);
        \path[-,draw,transform canvas={xshift=0.5em}, draw = blue,rounded corners]{} (phant13) -|        (gtr1);
        
        \path[line,transform canvas={yshift=0.5em}]{} (btr) --        (tht);
        
        \path[line,transform canvas={yshift=-0.5em},draw = red]{} (btr) --        (tht);
        
        \path[line,transform canvas={yshift=0.5em}]{} (tht) --        (gtr1);
        \path[line,transform canvas={yshift=-0.5em}, draw = red]{} (tht) --        (gtr1);

        %\path[-,draw, draw = blue]{} (phant32) --          (thtt.south);
        %\path[line, draw = blue,rounded corners]{} (phant32) -|        (gtr1.east);
        \path[-,draw, draw = blue]{} (phant32) --          (thtt.south);
        \path[line, draw = blue,rounded corners]{} (phant32) |-        (gtr1.east);
        
        
        %\path[line,transform canvas={xshift=-1.1em}]{} (phant33) --          (thtt.south);
        %\path[-,draw,transform canvas={xshift=-0.5em},rounded corners]{} (phant34) -|        (gtr1.east);
        \path[-,draw,transform canvas={yshift=0.5em},rounded corners]{} (phant34) |-        (gtr1.east);
        \path[line,transform canvas={xshift=-0.6em}]{} (phant33) --          (thtt.south);        
        
        \path[-,draw, draw = red,rounded corners]{} (wt1.south) |-          (phant31);
        \path[line, draw = red,rounded corners]{} (phant31) -|        (phant23);
        
        
        \path[line]{} (bval) --        (thtt);
        \path[line,transform canvas={yshift=-0.5em}]{} (thtt) --        (gtr2);
        \path[line,transform canvas={yshift=0.5em}, draw = blue]{} (gtr2) --        (thtt);
        
        \path[line,transform canvas={xshift=0.5em}, draw = red,rounded corners]{} (gtr1.south) |-        (tht1);

      \end{tikzpicture}%
}    
%
\vspace{0.5cm}
\underline{\hspace{ 5 in}}
\vspace{0.5cm}
%
  \begin{tikzpicture}[node distance=2.3cm]
  
    %\node[block, minimum height=2cm, text width=0.85cm,label={[align=left]above left:sample\\ weights}]                  (wt1){$w_{0,t-1}$ \\ $w_{1,t-1}$ \\ $w_{2,t-1}$ \\ \:\:\vdots \\ $w_{n,t-1}$};
    \node[block](wt_1){$w_{0,t-1}$};
    \node[block, below=0.55cm of wt_1](wt_2){$w_{1,t-1}$};
    \node[block, below=0.55cm of wt_2](wt_3){$w_{2,t-1}$};
    \node[block, below=0.55cm of wt_3](wt_4){$w_{3,t-1}$};
    
    \begin{scope}[on background layer]
    \node[fit={(wt_1) (wt_2)  (wt_3) (wt_4)}, draw,fill={blue!20},rounded corners] (wt1) {};
    \end{scope}
    
    \node[block, right of=wt1, minimum height=2cm, text width=0.85cm,label={[align=left]above right:training\\ samples}]                  (btr){\includegraphics[angle=0,origin=c,width=.85\textwidth]{figures/tikz/tr_set.png}};
    \node[below of=wt1,scale=0.05](phant1){}; 
    
    \node[block, right of=btr]   (tht){network \\ $\theta_{t-1}$};
    
    \node[block, right=1cm of phant2]   (gtr1){weighted loss \\ $\mathcal{L}_{\textrm{tr}}$};
    
    \node[right =1cm of gtr1,transform canvas={xshift=0.4em}]   (tht1){$\textcolor{red}{\theta_t}$};
    

    \path[line]{} (btr) --        (tht);
    \path[line]{} (tht) --        (gtr1);
    
    \path[-,draw,draw=blue]{} (wt1.south) --        (phant1);
    \path[line, rounded corners,draw=blue]{} (phant1) -|        (gtr1);
    \path[line]{} (gtr1) --        (tht1);
    

  \end{tikzpicture}%

%\caption{Meta learning update. $B_{\textrm{tr}}$, $B_{\textrm{val}}$ are training and validation batches. $w_{t-1}$ and $w_{t}$ are the training data weights at iteration $t-1$ and $t$. Likewise, $\theta_{t-1}$ and $\theta_{t}$ are the network parameters. $\alpha$ and $\beta$ are learning rates for the network parameter and training data updates respectively. The dotted line denotes the evaluation of $\nabla_w\mathcal{L}_{\textrm{val}}$ at $w_{t-1}$}
\caption{}
\label{fig:mml}
\end{figure}

\lily{Fig 1 is better than earlier one, but is still not straightforward to me... Another thing is it occupies too much space, ideally this graph is no more than half page. Maybe try powerpoint drawing? Didn't see Step 1}

==> figures/tikz/meta_update_phase2.tex <==
\begin{figure}
\centering
\scalebox{0.8}{
      \begin{tikzpicture}[node distance=2.3cm]
      
        \node[block, minimum height=2cm, text width=0.85cm,label={[align=left]above left:sample\\ weights}]                  (wt1){$w_{0,t-1}$ \\ $w_{1,t-1}$ \\ $w_{2,t-1}$ \\ \:\:\vdots \\ $w_{n,t-1}$};
        
        \node[block, right of=wt1, minimum height=2cm, text width=0.85cm,label={[align=left]above right:training\\ samples}]                  (btr){\includegraphics[angle=0,origin=c,width=.85\textwidth]{figures/tikz/tr_set.png}};
        
        \node[below of=wt1,scale=0.05](phant1){}; 
        
        \node[block, right of=btr]   (tht){network \\ $\theta_{t-1}$};
        
        \node[block, right=1cm of phant2]   (gtr1){[weighted] loss \\ $\mathcal{L}_{\textrm{tr}}$};
        
        \node[right =1cm of gtr1,transform canvas={xshift=0.4em}]   (tht1){$\textcolor{green}{\theta_t}$};
        

        \path[line]{} (btr) --        (tht);
        \path[line]{} (tht) --        (gtr1);
        
        \path[-,draw,draw=blue]{} (wt1.south) --        (phant1);
        \path[line, rounded corners,draw=blue]{} (phant1) -|        (gtr1);
        \path[line]{} (gtr1) --        (tht1);
        

      \end{tikzpicture}%
}    
\caption{}
\label{fig:mml}
\end{figure}

==> figures/tikz/mmupdate_bu.tex <==
\begin{figure}
\centering
\scalebox{0.8}{
      \begin{tikzpicture}[node distance=2.3cm]
        \node[block]                  (wt1){$w_{t-1}$};
        \node[right=0.5cm of wt1,scale=0.05](inv){};
        \node[decision, below of=wt1, label={above:{\small training data}}](btr){$B_{\textrm{tr}}$};
        \node[block, right= 2cm of wt1]   (gtr1){$\nabla_{\theta}\mathcal{L}_{\textrm{tr}}|_{\theta_t,w_{t-1}}$};
        \node[below=0.5cm of gtr1,scale=0.05](inv2){};
        \node[block, below of=gtr1]   (tht){$\theta_t$};        
        \node[block, below of=tht](gtr2){$\nabla_{\theta}\mathcal{L}_{\textrm{tr}}|_{\theta_t,w_t}$};
        \node[block, below of=gtr2, label={right:${\scriptstyle\theta_{t+1} = \theta_t - \alpha \nabla_{\theta}\mathcal{L}_{\textrm{tr}}|_{\theta_t,w_t}}$}]   (tht1){$\theta_{t+1}$};
        \node[block, right=4cm of gtr1, label={above:${\scriptstyle\theta_{\textrm{tmp}} = \theta_t - \alpha \nabla_{\theta}\mathcal{L}_{\textrm{tr}}|_{\theta_t,w_{t-1}}}$}]   (thtmp){$\theta_{\textrm{tmp}}$};
        \node[block,text width=2.5cm, below of=thtmp]   (gw){$\nabla_{w}\mathcal{L}_{\textrm{val}}|_{\theta_{\textrm{tmp}},w_{t-1}}$};        
        \node[decision, right of=gw, label={above:{\small validation data}}]   (bval){$B_{\textrm{val}}$};
        \node[block, left= 1cm of gw, label={above:${\scriptstyle w_{t} = w_{t-1} - \beta \nabla_{w}\mathcal{L}_{\textrm{val}}|_{\theta_{\textrm{tmp}},w_{t-1}}}$}]   (wt){$w_t$};         
        
        \path[line] (wt1) --          (gtr1);
        \path[-,draw]{} (btr) -|          (inv);
        \path[line] (inv) --          (gtr1);
        \path[line] (gtr1) --          (thtmp);
         \path[line] (thtmp) --          (gw);
        \path[line] (tht) --          (gtr1);
        
        \path[line] (bval) --          (gw);
        \path[line] (tht) --          (gtr2);
        \path[line] (gw) --          (wt);
        
        \path[dotted,draw] (gw) |-          (inv2);
        \path[dotted,draw] (inv2) -|          (wt1);
        
        \path[line] (btr) |-          (gtr2);
        \path[line] (wt) |-          (gtr2);
        \path[line] (gtr2) --          (tht1);
        

      \end{tikzpicture}%
}    
\caption{Meta learning update. $B_{\textrm{tr}}$, $B_{\textrm{val}}$ are training and validation batches. $w_{t-1}$ and $w_{t}$ are the training data weights at iteration $t-1$ and $t$. Likewise, $\theta_{t-1}$ and $\theta_{t}$ are the network parameters. $\alpha$ and $\beta$ are learning rates for the network parameter and training data updates respectively. The dotted line denotes the evaluation of $\nabla_w\mathcal{L}_{\textrm{val}}$ at $w_{t-1}$}
\label{fig:mml}
\end{figure}

==> figures/tikz/tlfowbu.tex <==
\begin{figure}
\centering
\scalebox{0.8}{
\begin{tikzpicture}[item/.style={circle,draw,thick,align=center},
itemc/.style={item,on chain,join}]
 \begin{scope}[start chain=going right,nodes=itemc,every
 join/.style={-latex,very thick},local bounding box=chain]
 
%\path node (A0) {$\theta_{t-k}$} node[xshift=2em] (A1) {$\theta_{t-2}$} node (A2) {$\theta_{t-1}$} node[minimum size=1cm] (At) {$\theta_t$};

\path node (A0) {$\theta_{t-k}$} node[xshift=1.5em,midway,scale=2,font=\bfseries,draw=none] {\dots} node (A1) {$\theta_{t-2}$};
\path (A1) node (A2) {$\theta_{t-1}$} node[minimum size=1cm] (At) {$\theta_t$};

 %\path (A1) -- node (A2) {$\theta_{t-1}$} node[midway,scale=2,font=\bfseries] {\dots};
 %\path (A2) node (At) {$\theta_t$};
 
 \end{scope}

 \node[above=2em of At,item, label={right:{$\scriptsize \bar{\theta} = \frac{1}{k+1}\sum_{i=0}^{k+1}\theta_i$}}] (AL) {$\bar{\theta}$};
 
 
  \foreach \X in {0,1,2,t} 
 {
 \draw[very thick,latex-] (AL) -- ++ (A\X);}
 
 
 \foreach \X/\Y in {0/k,1/2,2/1} 
 {
 \draw[very thick,latex-] (A\X.south) -- ++ (0,-2em)
 node[below,item,fill=gray!10] (x\X) {$w_{t-\Y}$};}
 
  \draw[very thick,latex-] (At.south) -- ++ (0,-2em)
 node[below,item,fill=gray!10, minimum size=1cm] (xt) {$w_{t}$};
 
 \path (x0) -- (x1) node[midway,scale=2,font=\bfseries] {\dots};
 
\end{tikzpicture}
}    


%
\caption{Training flow of our framework. Members of the $k$-member ensemble are trained sequentially on a common training set with weights $w$ using gradient descent. The training of one member is seeded by the preceding member in the ensemble. The network used at inference is an ensemble comprised of the last $k$ trained networks. The weights are computed so as to minimize the unweighted robust error on a validation set.}
\label{fig:frmwrk}
\end{figure}

==> figures/tikz/training_flow.tex <==
\iffalse
\begin{figure}
\centering
\scalebox{0.8}{
\begin{tikzpicture}[item/.style={circle,draw,thick,align=center},itemc/.style={item,on chain,join}]


 \begin{scope}[start chain=going right,nodes=itemc,every
 join/.style={-latex,very thick},local bounding box=chain]
 
%\path node (A0) {$\theta_{t-k}$} node[xshift=2em] (A1) {$\theta_{t-2}$} node (A2) {$\theta_{t-1}$} node[minimum size=1cm] (At) {$\theta_t$};

\path node (A0) {$\theta_{t-k}$} node[xshift=1.5em,midway,scale=2,font=\bfseries,draw=none] {\dots} node (A1) {$\theta_{t-2}$};
\path (A1) node (A2) {$\theta_{t-1}$} node[minimum size=1cm] (At) {$\theta_t$};

 %\path (A1) -- node (A2) {$\theta_{t-1}$} node[midway,scale=2,font=\bfseries] {\dots};
 %\path (A2) node (At) {$\theta_t$};
 
 \end{scope}

 \node[above=2em of At,item, label={right:{$\scriptsize \bar{\theta} = \frac{1}{k+1}\sum_{i=0}^{k+1}\theta_i$}}] (AL) {$\bar{\theta}$};
 
 
  \foreach \X in {0,1,2,t} 
 {
 \draw[very thick,latex-] (AL) -- ++ (A\X);}
 
 
 \foreach \X/\Y in {0/k,1/2,2/1} 
 {
 \draw[very thick,latex-] (A\X.south) -- ++ (0,-2em)
 node[below,item,fill=gray!10] (x\X) {$w_{t-\Y}$};}
 
  \draw[very thick,latex-] (At.south) -- ++ (0,-2em)
 node[below,item,fill=gray!10, minimum size=1cm] (xt) {$w_{t}$};
 
 \path (x0) -- (x1) node[midway,scale=2,font=\bfseries] {\dots};
 
\end{tikzpicture}
}    


%
\caption{Training flow of our framework. Members of the $k$-member ensemble are trained sequentially on a common training set with weights $w$ using gradient descent. The training of one member is seeded by the preceding member in the ensemble. The network used at inference is an ensemble comprised of the last $k$ trained networks. The weights are computed so as to minimize the unweighted robust error on a validation set.}
\label{fig:frmwrk}
\end{figure}
\fi 
\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/adveRoBoost_fig2_ver2.png}
    \caption{Training flow of our framework. Members of the $k$-member ensemble are trained sequentially on a common training set with weights $w$ using gradient descent. The training of one member is seeded by the preceding member in the ensemble. The network used at inference is an ensemble comprised of the last $k$ trained networks. The weights are computed so as to minimize the unweighted robust error on a validation set.}
    \label{fig:my_label}
\end{figure}


==> tables/ablation.tex <==
\begin{table}[h]
\caption{Ablation experiments: capacity of the axuiliary weight prediction network}
\label{tab:ablat_capacity}
\centering
\begin{tabular}{|l|l|l|l|}
\hline
\multirow{2}{*}{Capacity of $\omega$} &  \multicolumn{3}{l|}{CIFAR10} \\ \cline{2-4} 
                  & Clean           & PGD  & PGD - Clean             \\ \hline
$128$               &    86.1      &    58.9   & 27.2    \\ \hline \hline
$64$             &    83.6      &    57.4   & 26.2    \\ 
$64-64$             &    85.8     &   58.6  & 27.1  \\ 
$256$             &    85.7     &     57.7   &28     \\  \hline
\end{tabular}
\end{table}

\begin{table}[h]
\caption{Ablation experiments: TRADES coefficient $1/\lambda$}
\label{tab:ablat_lambda}
\centering
\begin{tabular}{|l|l|l|}
\hline
\multirow{2}{*}{$1/\lambda$} &  \multicolumn{2}{l|}{CIFAR10} \\ \cline{2-3} 
                  & Clean           & PGD               \\ \hline
$1/\lambda = 6$               &      86.1      &    58.9        \\ \hline \hline
$1/\lambda = 1$            &      87.4    &     52.5      \\ 
$1/\lambda = 5$              &    86.9    &    57.6   \\ 
$1/\lambda = 10$              &    83.8     &  57.9           \\  \hline
\end{tabular}
\end{table}

\begin{table}[h]
\caption{Ablation experiments: $\Delta$, input to the auxiliary network}
\label{tab:ablat_margin}
\centering
\begin{tabular}{|l|l|l|}
\hline
\multirow{2}{*}{$\Delta$} &  \multicolumn{2}{l|}{CIFAR10} \\ \cline{2-3} 
                  & Clean           & PGD               \\ \hline
$\Delta_{\textrm{multi-class}}$               &    86.1      &    58.9        \\ \hline \hline
$\Delta_{\textrm{class-unaware}}$             &  84.1        &    54.6       \\ 
$\hat{\ell}$             &  86.9       &  57.9     \\ 
$\hat{\ell} - \ell$             &  85.4       & 53.8            \\ \hline 
\end{tabular}
\end{table}


